Efficient Graph Field Integrators Meet Point Clouds

We present two new classes of algorithms for efficient field integration on graphs encoding point clouds. The first class, SeparatorFactorization(SF), leverages the bounded genus of point cloud mesh graphs, while the second class, RFDiffusion(RFD), uses popular epsilon-nearest-neighbor graph representations for point clouds. Both can be viewed as providing the functionality of Fast Multipole Methods (FMMs), which have had a tremendous impact on efficient integration, but for non-Euclidean spaces. We focus on geometries induced by distributions of walk lengths between points (e.g., shortest-path distance). We provide an extensive theoretical analysis of our algorithms, obtaining new results in structural graph theory as a byproduct. We also perform exhaustive empirical evaluation, including on-surface interpolation for rigid and deformable objects (particularly for mesh-dynamics modeling), Wasserstein distance computations for point clouds, and the Gromov-Wasserstein variant.

==> additional_experiments_main_paper.tex <==
% To be copied to the paper_experiments.tex
\section{Experiments on Point Cloud Classification}
\subsection{Topological Transformers}
We have complemented our additional experiments with results on Point Cloud Transformers (PCT)~\citep{Guo_2021}. The entrance point for the RFDiffusion algorithm is the topologically-modulated performized version~\citep{choromanski} of the regular PCT. The topological modulation works by Hadamard-multiplying regular attention matrix with the mask-matrix encoding relative distances between the points in the $3D$ space to directly impose structural priors while training the attention model. Performized PCT provides computational gains for larger point clouds ($N=2048$ points are used in our experiments). Moreover, its topologically modulated version can be executed in the favorable sub-quadratic time only if the mask-matrix itself supports sub-quadratic matrix-vector multiplication~\citep{topmasking} without the explicitly materialization of the attention and the mask matrices. RFDiffusion provides a low-rank decomposition via its novel RF-mechanism and the observation in Sec. 3.4 (~\citep{topmasking}), can be used for time-efficient training in our particular setting. We conduct our experiments on the ShapeNet dataset~\citep{Zhirong15CVPR}. Performized PCT with efficient RFDiffusion-driven masking achieves $\mathbf{91.13\%}$ validation accuracy and linear time complexity (due to the efficient integration algorithm with the RFDiffusion). The brute-force variant runs out of memory in training.

\subsection{Point Cloud Classification}~\label{sec:pc_expt}
We have also conducted point cloud classification experiments on ModelNet10~\citep{Zhirong15CVPR} and Cubes~\citep{meshcnn}, using our RFDiffusion kernel method. The classification in this case is conducted using the eigenvectors of the kernel matrix. Note that, as described in~\citep{nakatsukasa2019lowrank}, low-rank decomposition of the kernel matrix (provided directly by the RFDiffusion method via the random feature map mechanism) can be used to compute efficiently eigenvectors and the corresponding eigenvalues. For each dataset, we compute the $k$ smallest eigenvalues of the kernel matrix ($k = 32$ for ModelNet10 and $k = 16$ for Cubes). We pass these $k$ eigenvalues to a random forest classifier for downstream classification.  For all the experiments we use:  $\epsilon = .1$, $\lambda = -.1$ and we sample $2048$ points randomly for each shape in ModelNet. 

The brute-force baseline version for the ModelNet10 and Cubes explicitly constructs the epsilon-neighborhood graph, directly conducting the eigendecomposition of its adjacency matrix and exponentiating eigenvalues. Comparison with this variant is the most accurate apple-to-apple comparison. The baseline variant has time complexity $O(N^3)$ whereas our method for obtaining the eigenvectors is of time complexity $O(N)$. Our results are summarized in Table~\ref{tab:pc_classification}. Our method excels at these point cloud classification tasks, beating the brute-force  baseline method by almost $\mathbf{25}$ points on ModelNet10 and by $\mathbf{5}$ points on the Cubes. Our reported numbers are comparable to earlier methods on ModelNet (SPH and LFD achieving $79\%$~\citep{Zhirong15CVPR}). Cubes is a fairly challenging dataset and deep learning models like PointNet achieves only $55\%$ accuracy. 
% Note: 
% The RFD kernel produces a smoothened version of the epsilon-neighborhood graph, giving good results even when the baseline applying explicitly the epsilon-neighborhood graph does not. This is the case since random features replace the combinatorial object (a graph with edges and no-edges) with its “fuzzy” version, where all the nodes are connected by edges (that are not explicitly reconstructed though) but the weights corresponding to non-edges in the original graph are close to zero with high probability. This is yet another advantage of our proposed method.  

\begin{table}[h]
\caption{Point cloud classification using RFD Kernel}
\label{tab:pc_classification}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Dataset} & \textbf{\# Graphs}  & \textbf{\# Classes} & \textbf{Baseline} & \textbf{RFD} \\
\midrule
ModelNet10       & 3991/908                   & 10                  & 43                & $\mathbf{70}$       \\
Cubes            & 3759/659                   & 23                  & 39                & $\mathbf{44}$   \\
\bottomrule
\end{tabular}%
}
\end{table}
For additional experiments on graph classification, see section Appendix~\ref{sec:graph_classification}.



==> algorithms.tex <==
\section{Algorithms}
\label{sec:algorithms}

Our proposed method consists of two phases that we describe in detail below.

\paragraph{Mesh factorization:} The goal of this phase is to preprocess a graph in such a way that the approximate computation of $\mathbf{M}^{\mathrm{G},f}\mathbf{x}$ can be efficiently conducted.
We accomplish this by recursively factorizing the mesh-graph into sub-graphs via the balanced separator sub-procedure. We start by finding the separation $(A,B,S)$ of the graph with the balanced separator of size $|S|=o(\sqrt{|\mathrm{V}|})$ in time $T=O(|\mathrm{V}|\log(|\mathrm{V}|))$.
For every vertex $v \in A \cup B \cup S$, we record its shortest-path-distance
We then proceed recursively in the sub-graphs induced by $A$ and $B$. As a result of the mesh-factorization procedure, for every vertex $v \in \mathrm{V}(\mathrm{G})$ we obtain a vector . 

\subsection{Graph diffusion kernel weights and vector-graphs}

Let us now consider a modification of the Definition \ref{def:main}, where matrix $\mathbf{M} \in \mathbb{R}^{|\mathrm{V}| \times |\mathrm{V}|}$ is given as: $\mathbf{M}=\mathbf{M}^{\mathrm{G},\lambda}_{\mathrm{diff}} = \exp(\lambda \mathrm{Adj(\mathrm{G})})$, where
$\mathrm{Adj}(\mathrm{G}) \in \mathbb{R}^{|\mathrm{V}| \times |\mathrm{V}|}$ is the weighted adjacency matrix of weighted undirected graph $\mathrm{G}$ with a vector $\mathbf{n}_{i} \in \mathbb{R}^{d}$ assigned to a node $i$ for every $i \in \mathrm{V}$. We will assume furthermore that the weights $w_{i,j}$ satisfy for some known $f:\mathbb{R}^{d} \rightarrow \mathbb{R}$: 
\begin{equation}
w_{i,j}=f(\mathbf{n}_{i}-\mathbf{n}_{j})
\end{equation}
We call such graphs \textit{vector graphs}.
Assume that $\mathrm{Adj}(\mathrm{G})$ can be (approximately) decomposed as follows: $\mathrm{Adj}(\mathrm{G})=\mathbf{A}\mathbf{B}^{\top}$ for some $\mathbf{A},\mathbf{B} \in \mathbb{R}^{|\mathrm{V}| \times m}$ for some $m \ll |\mathrm{V}|$. Note that we have:
\begin{align}
\begin{split}
\exp(\lambda \mathbf{A}\mathbf{B}^{\top}) &= \sum_{i=0}^{\infty} \frac{1}{i!}(\lambda \mathbf{A}\mathbf{B}^{\top})^{i} \\
=
\mathbf{I}& + \sum_{i=0}^{\infty}\frac{1}{(i+1)!}\mathbf{A}(\lambda\mathbf{B}^{\top}\mathbf{A})^{i+1}\mathbf{A}^{-1} \\
= 
\mathbf{I}& + \mathbf{A}[\exp(\lambda \mathbf{B}^{\top}\mathbf{A}) - \mathbf{I}](\mathbf{B}^{\top}\mathbf{A})^{-1}\mathbf{B}^{\top}
\end{split}
\end{align}
The above formula provides a straightforward algorithms for the efficient multiplication $\mathbf{M}^{\mathrm{G},\lambda}_{\mathrm{diff}}\mathbf{x}$ for any $\mathbb{R}^{|\mathrm{V}|}$. 
Thus it remains to efficiently find the decomposition $(\mathbf{A},\mathbf{B})$ of $\mathrm{Adj}(\mathrm{G})$.
Assume that $w_{i,j}$ can be rewritten as: $w_{i,j} = \mathbb{E}[\phi(\mathbf{n}_{i})^{\top}\psi(\mathbf{n}_{j})]$
for some (randomized): $\phi, \psi: \mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$. Then it suffices to define the rows of $\mathbf{A}$ and $\mathbf{B}$ as: $\phi(\mathbf{n}_{i})^{\top}$ and $\psi(\mathbf{n}_{i})^{\top}$ respectively.

Below we show how to find mappings $\phi$ and $\psi$.
Note that we have:
\begin{align}
\begin{split}
f(\mathbf{z}) &= \int_{\mathbb{R}^{3}} \exp(2 \pi i \omega^{\top}\mathbf{z})\tau(\omega)d(\omega)\\
&= \int_{\mathbb{R}^{3}} \exp(2 \pi i \omega^{\top}\mathbf{z})\frac{\tau(\omega)}{p(\omega)}p(\omega) d(\omega),    
\end{split}
\end{align}
where $\tau: \mathbb{R}^{d} \rightarrow \mathbb{C}$ is the Fourier Transform (FT) of $f$ and $p$ is a pdf function corresponding to some probabilistic distribution $P \in \mathcal{P}(\mathbb{R}^{d})$.

Then we can define for $\omega_{1},\ldots,\omega_{s} \sim P$ and $\nu_{i}=\sqrt{\frac{\tau(\omega_{i})}{p(\omega_{i})}}$.:
\begin{equation}
\phi(\mathbf{v}) = \frac{1}{\sqrt{s}} 
\left(\exp(2 \pi i \omega_{1}^{\top}\mathbf{v})\nu_{1},\ldots,\exp(2 \pi i \omega_{s}^{\top}\mathbf{v})\nu_{s}\right)^{\top}
\end{equation}
\begin{equation}
\psi(\mathbf{v}) = \frac{1}{\sqrt{s}} 
\left(\exp(-2 \pi i \omega_{1}^{\top}\mathbf{v})\nu_{1},\ldots,\exp(-2 \pi i \omega_{s}^{\top}\mathbf{v})\nu_{s}\right)^{\top}
\end{equation}


\textbf{Note:} Distribution $P$ should be in general chosen to minimize the variance of the above unbiased estimator of $f(z)$, but of course should also provide efficient sampling mechanism. 

\subsubsection{Special instantiation of a function $f$}

\textbf{Case 1:} $f(\mathbf{z})=1$ if $\|\mathbf{z}\|_{1} \leq \epsilon$ and $f(\mathbf{z})=0$ otherwise.

In that setting we have:
\begin{equation}
\tau(\mathbf{\xi}) = \prod_{i=1}^{d} \frac{\mathrm{sin}(2\epsilon \xi_{i})}{\xi_{i}}
\end{equation}

\textbf{Case 2:} $f(\mathbf{z})=1$ if $\|\mathbf{z}\|_{2} \leq \epsilon$ and $f(\mathbf{z})=0$ otherwise.
In that case $\tau$ is the $d$th order \textit{Bessel function}.


==> bin.tex <==
For $u,v y edge \in V(T)$, we say that $\mathcal{D}$ is $(u,v)$-{\em safe} if for every $x,y \in B_v$ there is a path in $G$ between $x$ and $y$ not passing through any vertex in $B_u \setminus B_v$. We say that $\mathcal{D}$ is {\em safe} if it is $(u,v)$-safe for every $\{u,v\} \in E(T)$. 

For every $x,y \in V(G)$, fix a paths $P_{x,y}$ between $x$ and $y$ of langth $dist_G(x,y)$. For a natural number $\ell$, we write 

$$B_v^\ell = \bigcup_{x,y \in B_v, \; dist_G(x,y)< \ell} V(P_{x,y}) \; .$$

It is easy to see that 

\begin{theorem}
    The sets $B_v^\ell$ form a tree-decomposition.
\end{theorem}

\begin{theorem}
    If $\mathcal{D}$ is safe then either $G[B_v^\ell]$ is connected for all $v \in V(T)$, or $G$ has a geodesic cycle of length at least $2\ell$. 
\end{theorem}

For $\{u,v\} \in E(T)$, we say that $(u,v)$ is {\em ready} in $\mathcal{D}$ if $(v,w)$ is safe for every neighbor $w$ of $v$ other than $u$. We obtain an auxiliary graph $A_v$ on $B_v$, starting from the induced graph $G[B_v]$, and then adding a clique on $B_w \cap B_v$ for every $T$-neighbor $w \neq u$ of $v$. Let $C_1, \ldits, C_j$ be the connected componnents of $A_v$. We construct a new tree $T'$ obtained from $T$ by deleting $v$ and adding $j$ new vertices $v_1, \ldots, v_j$. We connect $u$ with an edge to all of $v_1, \ldots, v_j$, and for every $T$-neighbor $w \neq u$ of $v$ we connect $w$ to $v_i$ if and only if $B_w \cap C_i \neq \emptyset$. We set $B_{v_i} = C_i$. It is easy to check that $T'$ is a tree yielding a tree-decomposition with the bags $(B_t: t \in V(T))$. We call this process a {\em check} on $(u,v)$. If $j=1$ then we say that the check is {\em passive}, and if $j>1$ then we say that the check is {\em active} and the vertex $v$ {\em splits} in it to $j$ vertices. 

By applying this process again and again whenever there exists $(u,v)$ which is ready but not safe, we can get a safe tree-decomposition. Note that if we a tree-decomposition $\mathcal{D}$ on a tree $T$ with $L$ vertices, where every bag has size at most $k$, then every vertex splits to at most $k$ vertices. Therefore if eventually, we get a tree-decomposition $\mathcal{D}'$ on a tree $T'$, then $|V(T')| \leq kL$. There are at most $2|E(T')| < 2kL$ passive checks and at most $|V(T')| \leq kL$ active checks, so altogether there are less than $3kL$ checks. 

The process of calculating the auxiliary graph, if conducted naively might have a time complexity of more than a function of $k$. However, this can be remedied if before starting the process we check for every $T$-vertex $v$ and every two vertices $x,y \in B_v$, whether $\{x,y\}$ is contained in zero, one, or more than one bags $B_w$, where $w$ is a $T$-neighbor of $v$. after this pre-processing, the auxiliary graph in each check can be calculated in $O(k^2)$ time. To sum up, we get the following. 

\begin{theorem}
    Let $G$ be a finite connected undirected graph and let $\mathcal{D} = (T,(B_v: v \in V(T)))$ be a tree-decomposition of $G$ with $L$ vertices, where each bag has size at most $k$. Then there is an algorithm with time complexity $O(Lk^3)$ for obtaining a safe tree decomposition of $G$, where still each bag has size at most $k$. 
\end{theorem}


If for some $w \in V(T')$ and some $s,t \in X'_w$ we have $dist_G(s,t) \geq \ell$, then there is a geodesic cycle in $G$ of length at least $2 \ell$. Therefore we may assume $dist_G(s,t) < \ell$.
